On the Usefulness of the Fit-on-the-Test View on Evaluating Calibration of Classifiers

Every uncalibrated classifier has a corresponding true calibration map that calibrates its confidence. Deviations of this idealistic map from the identity map reveal miscalibration. Such calibration errors can be reduced with many post-hoc calibration methods which fit some family of calibration maps on a validation dataset. In contrast, evaluation of calibration with the expected calibration error (ECE) on the test set does not explicitly involve fitting. However, as we demonstrate, ECE can still be viewed as if fitting a family of functions on the test data. This motivates the fit-on-the-test view on evaluation: first, approximate a calibration map on the test data, and second, quantify its distance from the identity. Exploiting this view allows us to unlock missed opportunities: (1) use the plethora of post-hoc calibration methods for evaluating calibration; (2) tune the number of bins in ECE with cross-validation. Furthermore, we introduce: (3) benchmarking on pseudo-real data where the true calibration map can be estimated very precisely; and (4) novel calibration and evaluation methods using new calibration map families PL and PL3.

==> temp.tex <==
% Cut from intro for related work

Several different solutions to this problem have been proposed: e.g. using kernel based estimates \citep{Widmann2019CalibrationTI,Zhang2020MixnMatchEA}, or choosing the maximal number of bins which leads to a monotonically increasing reliability diagram \citep{sweep}.
More broadly, evaluation of calibration has been the main focus of several works:
%\citet{murphy1977reliability} use reliability diagrams for estimating the trustworthiness of precipitation probability forecasts.
\citet{vaicenavicius2019evaluating} proposed a more general definition of calibration and proposed a method to perform statistical tests of calibration, based on binning.
\citet{Widmann2019CalibrationTI} proposed the kernel calibration error for calibration evaluation in multi-class classification.
%\citet{sweep} proposed to sweep from 1 bin towards more bins until the last number of bins before the reliability diagram becomes non-monotonic.

%We suggest to view calibration by what we call the fit-on-test paradigm, introduced in Section~\ref{sec:fit_on_the_test}. 
%This allows to use post-hoc calibration methods as calibration evaluators and vice versa, and also shows that cross-validation can be used for choosing the number of bins in ECE. 
%In Section~\ref{sec:eval_methods_of_cal}, we go into evaluation methods of calibrators and evaluation of calibration evaluators.
%In Section~\ref{sec:related_work}, we discuss related work and application to multi-class.
%In Section~\ref{sec:PL_RD}, we give details about our proposed piecewise linear methods and the usefulness of the logit-logit space.
%In Section~\ref{sec:experiments}, we present results on pseudo-real data and  conclude in Section~\ref{sec:conclusion}.

%\subsection{Related Work}

%\TO{ see peatükk vaja üle vaadata}
The research on evaluating calibration has gone hand-in-hand with the research on post-hoc calibration,  which aims to learn a calibration map transforming the classifier's output probabilities into calibrated probabilities.
Many papers contributed to both post-hoc calibration and evaluation:
\citet{naeini2015} proposed BBQ and used ECE to evaluate calibration; % \TO{REF-Naeini2015}
\citet{Guo2017} proposed temperature, vector and matrix scaling, and used the reliability diagrams and ECE for evaluating confidence in multi-class classification.
\citet{kumar2019neurips} proposed scaling-binning calibration, a new debiasing method for ECE and the notion of marginal calibration error.
\citet{Kull2019BeyondTS} proposed Dirichlet calibration and the notion of classwise-calibration error.
\citet{Zhang2020MixnMatchEA} proposed generic Mix-n-Match calibration strategies and used kernel density estimation (KDE) for estimating CE.
\inserted{\citet{spline_gupta21} proposed a calibration evaluation metric based on the Kolmogorov-Smirnov test and a calibration method based on fitting splines.}
%\inserted{\citet{IOP_rahimi20} proposed ...}  
